PixT3: Pixel-based Table-To-Text Generation

Table-to-text generation involves generating appropriate textual descriptions given structured tabular data. It has attracted increasing attention in recent years thanks to the popularity of neural network models and the availability of large-scale datasets. A common feature across existing methods is their treatment of the input as a string, i.e., by employing linearization techniques that do not always preserve information in the table, are verbose, and lack space efficiency. We propose to rethink data-to-text generation as a visual recognition task, removing the need for rendering the input in a string format. We present PixT3, a multimodal table-to-text model that overcomes the challenges of linearization and input size limitations encountered by existing models. PixT3 is trained with a new self-supervised learning objective to reinforce table structure awareness and is applicable to open-ended and controlled generation settings. Experiments on the ToTTo and Logic2Text benchmarks show that PixT3 is competitive and, in some settings, superior to generators that operate solely on text.

==> sec/5_analysis.tex <==
\section{Analysis and discussion}



\subsection{Qualitative analysis}
\label{sec:qualitative_analysis}

Faithfulness
Thanks to this analysis we see that the no-highlighted model captures the tendencies of information distribution in tables. With a distribution of mentioned tables being:

Qualitative analysis.
- Mention insights gathered, how models tend to reference cells in the right side of the table following the highlight distribution and common human-western conventions of relevant information positioning.


\subsection{Large vs base PixT3}

maybe 282M parameters are enough to capture the requirements for the task of Table-to-Text and adding more parameters is only needed to capture multiple tasks at once? (Nah, I don't think so)

% more
Excluding the table from the input converts the task of controlled
Table-to-Text to a fundamental text parsing operation. It is
reasonable to remove potentially noisy information form the input,
however, doing so makes models vulnerable to


%%% Local Variables: 
%%% mode: latex
%%% TeX-master:  "../manuscript"
%%% End:


==> sec/9_acknowledgements.tex <==
\section*{Acknowledgements}
We thank the meta-reviewer and anonymous reviewers for their constructive feedback. The authors also thank \aclfinal{is there someone?} for insightful comments on earlier versions of this work. We gratefully acknowledge the support of the UK Engineering and Physical Sciences Research Council (grant
EP/L016427/1).
